Falling balls in a viscous fluid with contact: Comparing numerical simulations with experimental data

We evaluate a number of different finite element approaches for fluid-structure (contact) interaction problems against data from physical experiments. For this we take the data from experiments by Hagemeier [Mendeley Data, doi: 10.17632/mf27c92nc3.1]. This consists of trajectories of single particles falling through a highly viscous fluid and rebounding off the bottom fluid tank wall. The resulting flow is in the transitional regime between creeping and turbulent flows. This type of configuration is particularly challenging for numerical methods due to the large change of the fluid domain and the contact between the wall and particle. In the numerical simulations we consider both rigid body and linear elasticity models for the falling particles. In the first case, we compare results obtained with the well established Arbitrary Lagrangian Eulerian (ALE) approach and a moving domain CutFEM method together with a simple and common approach for contact avoidance. For the full fluid-structure interaction (FSI) problem with contact, we use a fully Eulerian approach in combination with a unified FSI-contact treatment using Nitsche's method. For higher computational efficiency we use the geometrical symmetry of the experimental set up to reformulate the FSI system into two spatial dimensions. Finally, we show full three dimensional ALE computations to study the effects of small perturbations in the initial state of the particle to investigate deviations from a perfectly vertical fall observed in the experiment. The methods are implemented in open-source finite element libraries and the results are made freely available to aide reproducibility.

==> files/definitions.tex <==
% Environments & Visual--------------------------------------------------------

% Tables and figures
\AtBeginEnvironment{tabular}{\footnotesize}
%\numberwithin{table}{section}

\makeatletter
\renewcommand{\fps@figure}{tp}
\renewcommand{\fps@table}{tp}
\makeatother

% Modify font
\makeatletter
\renewcommand\paragraph{%
  \@startsection{paragraph}
    {4}
    {\z@}
    {3.25ex \@plus1ex \@minus.2ex}
    {-1em}
    {\normalfont\sectfont\normalsize\bfseries\maybe@addperiod}%
}
\newcommand{\maybe@addperiod}[1]{%
  #1\@addpunct{.}%
}
\makeatother

\renewcommand*{\mkbibnamefamily}[1]{\textsc{#1}}
\renewcommand*{\mkbibnamegiven}[1]{\textsc{#1}}
\renewcommand*{\mkbibnameprefix}[1]{\textsc{#1}}
\renewcommand*{\mkbibnamesuffix}[1]{\textsc{#1}}

\setkomafont{caption}{\sffamily\small}
\setkomafont{captionlabel}{\bfseries\usekomafont{caption}}
\captionsetup[subfloat]{font={small, sf}}

% Math statement environments
\numberwithin{equation}{section}
\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}
\newcounter{theorems}
\numberwithin{theorems}{section}

\theoremstyle{plain}
\newtheorem{theorem}[theorems]{Theorem}
\newtheorem{lemma}[theorems]{Lemma}
\newtheorem{proposition}[theorems]{Proposition}
\newtheorem{corollary}[theorems]{Corollary}

\theoremstyle{definition} 
\newtheorem{definition}[theorems]{Definition}
\newtheorem{problem}{Problem}
\renewcommand\theproblem{P\arabic{problem}}
\newtheorem{assumption}{Assumption}
\renewcommand\theassumption{A\arabic{assumption}}
\newtheorem*{notation}{Notation}

\theoremstyle{remark} 
\newtheorem*{remark}{Remark}
\newtheorem{remnum}[theorems]{Remark}
\newtheorem{example}[theorems]{Example}

\makeatletter
\renewcommand*\thmhead[3]{\thmname{#1}\thmnumber{ #2}\thmnote{ ({\itshape#3})}}
\makeatother

% Link colouring
\definecolor{darkred}{RGB}{139,0,0}
\definecolor{mediumblue}{RGB}{0,0,205}
\definecolor{forestgreen}{RGB}{34,139,34}

\hypersetup{%
  linkcolor=darkred,%
  urlcolor=forestgreen,%
  citecolor=mediumblue%
}

% Plot settings ---------------------------------------------------------------
\pgfplotsset{every axis/.append style={
                title style = {font=\footnotesize},
                legend style = {font=\footnotesize},
                label style = {font=\footnotesize},
                tick label style = {font=\footnotesize},
                axis line style = {line width=.7pt},
                legend style = {line width=.7pt, cells = {line width = 1pt}},
                line width=1pt,
                mark options={solid},
                tickpos=left,
                tick style = {semithick},
                cycle list={[samples of colormap={6 of viridis}]},
                }
}


% Definitions------------------------------------------------------------------

% Sets
\newcommand{\R}{\mathds{R}}							% Set of real numbers
\newcommand{\N}{\mathds{N}}							% Set of natural numbers
\newcommand{\PP}{\mathbb{P}}
\renewcommand{\P}[2]{\PP^{#1}(#2)}					% Set of Polynomials
\newcommand{\E}{\pazocal{E}^\mathbb{P}}				% Polynomial extension to R^d

% Sobolev and Lebesgue spaces
\renewcommand{\L}[2]{\pazocalbf{L}^{#1}(#2)}		% Vec. val. Lebesgue space
\newcommand{\Linf}[1]{\L{\infty}{#1}}				% Vector valued L-infinity
\newcommand{\Ltwozero}[1]{\pazocal{L}^2_0(#1)}		% Scalar L2 with zero mean
\renewcommand{\H}[3]{\pazocalbf{H}^{#1}_{#2}(#3)}	% Vec.-val. Sobolev H space  

% Products and norms		
\newcommand{\dual}[3]{\langle #1, #2\rangle_{#3}}	% Duality pairing 
\newcommand{\lprod}[3]{(#1,#2)_{#3}}				% L2 inner product
\newcommand{\nrm}[2]{\Vert#1\Vert_{#2}}				% Norm

% Domains
\renewcommand{\O}{\Omega}							% Domain Omega
\newcommand{\Ot}{\widetilde{\O}}					% Background Domain
\newcommand{\G}{\Gamma}								% Domain boundary

\newcommand{\FL}{\pazocal{F}}						% Fluid region
\newcommand{\SO}{\pazocal{S}}						% Solid region
\newcommand{\IN}{\pazocal{I}}						% Fluid-Solid interface

\newcommand{\Gtop}{\G_\text{top}}
\newcommand{\Gbot}{\G_\text{bottom}}
\newcommand{\Gwall}{\G_\text{wall}}

% Meshes
\newcommand{\T}{\mathcal{T}}
\newcommand{\Th}{\T_h}								% Mesh
\newcommand{\Fh}{\mathcal{F}_h}						% Set of g-p facets
\newcommand{\hmax}{h_\text{max}}
\newcommand{\hmin}{h_\text{min}}

% Finite element spaces
\newcommand{\V}{\bm{V}}	
\newcommand{\W}{\bm{W}}	
\newcommand{\Z}{\bm{Z}}								% Velocity function space

% Finite element functions
\renewcommand{\u}{\bm{u}}	
\newcommand{\z}{\bm{z}}						        % Vector valued velocity
\newcommand{\uf}{\mathfrak{u}}						% Coeffs of FEM function
\let\vs\v
\renewcommand{\v}{\bm{v}}							% Vec. val. test function
\newcommand{\omegat}{\bm{\omega}}					% Vec. val. rotation

\renewcommand{\d}{\bm{d}}                           % Solid displacement
\renewcommand{\c}{\bm{c}} 

\newcommand{\w}{\bm{w}}								% Vector valued function
\newcommand{\bb}{\bm{\beta}}						% Convection velocity
\newcommand{\n}{\bm{n}}								% Normal vector
\newcommand{\x}{\bm{x}}								% Coordinate vector
\newcommand{\f}{\bm{f}}								% Forcing vector

% Operators
\newcommand{\Ex}{\pazocal{E}}						% Extension operator
\newcommand{\restr}[2]{{%
  \left.\kern-\nulldelimiterspace#1\right|_{#2}}}	% Restriction operator
\newcommand{\jump}[1]{\llbracket #1 \rrbracket }    % Jump

% Named math operators
\DeclareMathOperator{\meas}{meas}					% measure
\DeclareMathOperator{\Id}{Id}						% Identity
\DeclareMathOperator{\diver}{div}					% Divergence
\renewcommand{\div}{\diver}
\DeclareMathOperator{\dist}{dist}					% Distance
\DeclareMathOperator{\trace}{tr}					% Trace
\DeclareMathOperator*{\esssup}{ess\,sup}			% Essential supremum
\DeclareMathOperator{\vol}{vol}

% Fluid (-Structure Interaction)
\newcommand{\stress}{\bm{\sigma}(\u,p)}				% Cauchy stress tensor
\newcommand{\sstress}{\bm{\sigma}_s}

% Miscellaneous
\newcommand{\nf}[2]{\nicefrac{#1}{#2}}
\newcommand{\eps}{\varepsilon}						% Epsilon shorthand
\newcommand{\dt}{\Delta t}							% Time-step
\newcommand{\st}{\;\vert\;}							% Set "such that"


